POTATO: The Portable Text Annotation Tool

We present POTATO, the Portable text annotation tool, a free, fully open-sourced annotation system that 1) supports labeling many types of text and multimodal data; 2) offers easy-to-configure features to maximize the productivity of both deployers and annotators (convenient templates for common ML/NLP tasks, active learning, keypress shortcuts, keyword highlights, tooltips); and 3) supports a high degree of customization (editable UI, inserting pre-screening questions, attention and qualification tests). Experiments over two annotation tasks suggest that POTATO improves labeling speed through its specially-designed productivity features, especially for long documents and complex tasks. POTATO is available at https://github.com/davidjurgens/potato and will continue to be updated.

==> comparison-table-wide.tex <==

\begin{table*}[t!]
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\centering

\resizebox{\textwidth}{!}{
   \rowcolors{3}{}{lightgray}
   
   % TODO Fix the centering and alignment with https://texblog.org/2019/06/03/control-the-width-of-table-columns-tabular-in-latex/
    \begin{tabular}{r |
    P{1.4cm} c c P{1.5cm} p{1.2cm} c P{1.3cm}
    | 
    P{1.5cm} P{1.5cm} P{2.0cm} P{1.5cm}
    |
    P{1.5cm} P{2.0cm} P{1.5cm}
    | 
    P{1.3cm}
    | c | P{1cm} }
 \multicolumn{1}{c}{} & \multicolumn{7}{c}{\textbf{Flexibility}} & \multicolumn{4}{c}{\textbf{Productivity}} & \multicolumn{3}{c}{\textbf{Surveyflow}} & \multicolumn{1}{c}{\textbf{Privacy}} & \multicolumn{2}{c}{\textbf{Price and Availability}} 
 \\ \cline{2-18}
 
 & Multi Scheme & Multimodal & Span & Multilingual Multi-domain &  Many Labels & Templates & Editable UI 
 & Automatic task assignment & Active learning & Conditional Highlighting & Keyboard shortcut
 & Prestudy test & Attention test & Survey questions
 & Runs Locally  
 & Price & Open-source 
 \\ \cline{1-18}
 
%                MT       MM      SP      MTL      ML       Tmp      UI      ATA     AL        CH      KeyS     PT        AT       SQ      Loc      $         OS
Label Studio & \cmark & \cmark &       &       & \cmark & \cmark & \cmark &        &        &        & \cmark &        &        &        & \cmark & Free  & \cmark \\ \hline
Doccano      &        & \cmark &       &       & \cmark &        &        &        &        &        & \cmark &        &        &        & \cmark & Free  & \cmark \\ \hline
FLAT         &        &        &       &       & \cmark &        & \cmark &        &        &        &        &        &        &        & \cmark & free  & \cmark \\ \hline
LightTag     & \cmark & \cmark &       &       & \cmark & \cmark &        &        &        &        & \cmark &        &        &        &        & Free for academia &  \\ \hline
Prodigy      &        & \cmark &       &       &        & \cmark &        &        & \cmark &        & \cmark &        &        &        & \cmark & \$390 &  \\ \hline
Tagtog       & \cmark &        &       &       & \cmark & \cmark &        &        &        &        &        &        &        &        & \cmark & \$59/person-month &  \\ \hline
%FITAnnotator &        &        &        & \cmark &        & \cmark &        &        & \cmark & Not available &  \\ \hline
\potato      & \cmark & \cmark &       & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark \\ \hline

    \end{tabular}}
    \caption{Comparisons between \potato and other text annotation systems over four themes. %Potato provides free text annotation solutions with flexibility for diverse needs, a series of productivity features as well as privacy-reserving designs. 
    % \daj{to-do: fix the vertical bars disappearing due to the new cmark macro centering.}
    \jp{add compatibility with AMT and prolific, behavioral tracking}
    }
    \label{tab:comparisons}
\end{table*}

